A branch-and-cut algorithm for vehicle routing problems with three-dimensional loading constraints

This paper presents a new branch-and-cut algorithm based on infeasible path elimination for the three-dimensional loading capacitated vehicle routing problem (3L-CVRP) with different loading problem variants. We show that a previously infeasible route can become feasible by adding a new customer if support constraints are enabled in the loading subproblem and call this the incremental feasibility property. Consequently, different infeasible path definitions apply to different 3L-CVRP variants and we introduce several variant-depending lifting steps to strengthen infeasible path inequalities. The loading subproblem is solved exactly using a flexible constraint programming model to determine the feasibility or infeasibility of a route. An extreme point-based packing heuristic is implemented to reduce time-consuming calls to the exact loading algorithm. Furthermore, we integrate a start solution procedure and periodically combine memoized feasible routes in a set-partitioning-based heuristic to generate new upper bounds. A comprehensive computational study, employing well-known benchmark instances, showcases the significant performance improvements achieved through the algorithmic enhancements. Consequently, we not only prove the optimality of many best-known heuristic solutions for the first time but also introduce new optimal and best solutions for a large number of instances.

==> tikzlibrarydubins.code.tex <==
%%
%% This is file `tikzlibrarydubins.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% sankey.dtx  (with options: `tikzlibrarydubins.code.tex')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2016, 2021 by Paul Gaborit
%% 
%% This work may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License, either version 1.3 of this license or (at
%% your option) any later version.  The latest version of this license is
%% in
%% 
%% <http://www.latex-project.org/lppl.txt>
%% 
%% and version 1.3 or later is part of all distributions of LaTeX version
%% 2005/12/01 or later.
%% 
%% This work has the LPPL maintenance status “maintained”.
%% 
%% The Current Maintainer of this work is Paul Gaborit.
%% 
%% This work consists of the files sankey.dtx, sankey.ins and the derived
%% files sankey.sty, tikzlibrarydubins.code.tex, sankey-doc-preamble.sty,
%% sankey-example1.tex, sankey-example2.tex, sankey-example3.tex,
%% sankey-example3-variation.tex, sankey-example4.tex,
%% sankey-example-energy.tex
%% 
\def\tikzlibrarydubins@version{v3.0.1}
\def\tikzlibrarydubins@date{2022/02/04}
\usetikzlibrary{calc}
\RequirePackage{etoolbox}
\RequirePackage{xfp}

\newbool{dubinspathreverse}
\def\ifpgfmathcond#1{%
  \pgfmathparse{(#1)?1:0}%
  \ifnumequal{\pgfmathresult}{1}%
}
\def\dbp@getxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone(#3)\relax%
  \edef#1{\the\pgf@x}%
  \edef#2{\the\pgf@y}%
}
\def\dbp@anglebetween#1#2#3{%macro, s, t
  \dbp@getxy\dbp@ax\dbp@ay{#2}
  \dbp@getxy\dbp@bx\dbp@by{#3}
  \pgfmathsetmacro#1{atan2(\dbp@by-\dbp@ay,\dbp@bx-\dbp@ax)}
}
\def\dbp@distancebetween#1#2#3{%macro, s, t
  \dbp@getxy\dbp@ax\dbp@ay{#2}
  \dbp@getxy\dbp@bx\dbp@by{#3}
  \edef#1{\fpeval{sqrt(%
      (\dbp@bx-\dbp@ax)*(\dbp@bx-\dbp@ax)%
      +(\dbp@by-\dbp@ay)*(\dbp@by-\dbp@ay)%
      )}}%
}
\newcommand\dbp@rsr{% s, sa, t, ta, as, len, at, r
  let
  \p{tr}=([shift={(\dbp@angb-90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga+90},
  \n2={\dbp@angb+90},
  \n3={\n2+\dbp@lastangle}
  in
  arc(\n1:\n1-\dbp@firstangle:\dbp@rradius pt)
  -- ([shift={(\p{tr})}]\n3:\dbp@rradius pt)
  arc(\n3:\n2:\dbp@rradius pt)
}
\newcommand\dbp@lsl{% s, sa, t, ta, as, len, at, r
  let
  \p{tl}=([shift={(\dbp@angb+90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga-90},\n2={\n1+\dbp@firstangle},
  \n3={\dbp@angb-90},\n4={\n3-\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@lradius pt)
  -- ([shift={(\p{tl})}]\n4:\dbp@lradius pt)
  arc(\n4:\n3:\dbp@lradius pt)
}
\newcommand\dbp@rsl{% s, sa, t, ta, as, len, at, r
  let
  \p{tl}=([shift={(\dbp@angb+90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga+90},\n2={\n1-\dbp@firstangle},
  \n3={\dbp@angb-90},\n4={\n3-\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@rradius pt)
  -- ([shift={(\p{tl})}]\n4:\dbp@lradius pt)
  arc(\n4:\n3:\dbp@lradius pt)
}
\newcommand\dbp@lsr{% s, sa, t, ta, as, len, at, r
  let
  \p{tr}=([shift={(\dbp@angb-90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga-90},\n2={\n1+\dbp@firstangle},
  \n3={\dbp@angb+90},\n4={\n3+\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@lradius pt)
  -- ([shift={(\p{tr})}]\n4:\dbp@rradius pt)
  arc(\n4:\n3:\dbp@rradius pt)
}
\newcommand\dbp@lrl{% s, sa, t, ta, as, ai, at, r
  let
  \n1={\dbp@anga-90},\n2={\n1+\dbp@firstangle},
  \n3={\dbp@angb-90},\n4={\n3-\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@lradius pt)
  arc(\n2+180:\n2+180-\dbp@midparam:\dbp@rradius pt)
  arc(\n4:\n3:\dbp@lradius pt)
}
\newcommand\dbp@rlr{% s, sa, t, ta, as, ai, at, r
  let
  \n1={\dbp@anga+90},\n2={\n1-\dbp@firstangle},
  \n3={\dbp@angb+90},\n4={\n3+\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@rradius pt)
  arc(\n2+180:\n2+180+\dbp@midparam:\dbp@lradius pt)
  arc(\n4:\n3:\dbp@rradius pt)
}
\newcommand\dbp@rev@lsl{\dbp@rsr}
\newcommand\dbp@rev@rsr{\dbp@lsl}
\newcommand\dbp@rev@lsr{\dbp@lsr}
\newcommand\dbp@rev@rsl{\dbp@rsl}
\newcommand\dbp@rev@lrl{\dbp@rlr}
\newcommand\dbp@rev@rlr{\dbp@lrl}
\newcommand\dubinspath[1]{%
  \pgfextra{
    \dubinspathset{#1}
    \ifbool{dubinspathreverse}{
      \edef\dbp@newa{\dbp@b}
      \edef\dbp@newb{\dbp@a}
      \pgfmathsetmacro\dbp@newanga{180+\dbp@angb}
      \pgfmathsetmacro\dbp@newangb{180+\dbp@anga}
      \edef\dbp@newfirstangle{\dbp@lastangle}
      \edef\dbp@newlastangle{\dbp@firstangle}
      \edef\dbp@newmethod{rev@\dbp@method}
      \edef\dbp@newlradius{\dbp@rradius}
      \edef\dbp@newrradius{\dbp@lradius}
      \dubinspathset{
        start point=\dbp@newa,
        end point=\dbp@newb,
        start angle=\dbp@newanga,
        end angle=\dbp@newangb,
        first angle=\dbp@newfirstangle,
        last angle=\dbp@newlastangle,
        left and right minimum radii=\dbp@newlradius pt and \dbp@newrradius pt,
        method=\dbp@newmethod,
      }
    }{}
  }
  \csname dbp@\dbp@method\endcsname%
}
\def\dbp@store#1#2{%
  \expandafter\xdef\csname dbp@store@#1@#2\endcsname%
  {\csname dbp@#2\endcsname}%
}
\def\dbp@get#1#2{%
  \csname dbp@store@#1@#2\endcsname%
}
\def\dbp@setparams#1#2#3#4#5{%
  % method, length, fisrt angle, middle param, last angle
  \edef\dbp@method{#1}
  \edef\dbp@length{#2}
  \edef\dbp@firstangle{#3}
  \edef\dbp@middleparam{#4}
  \edef\dbp@lastangle{#5}
  \ifdef{\dbp@storename}{
    \foreach \p in {method,length,firstangle,middleparam,lastangle}{
      \dbp@store{\dbp@storename}{\p}
    }
  }{}
}
\def\dbp@updateparams#1#2#3#4#5{
  \ifpgfmathcond{#2<\dbp@length}{
    \dbp@setparams{#1}{#2}{#3}{#4}{#5}
  }{}
}
\tikzset{
  dubins path/.is family,
  dubins path,
  start point/.store in=\dbp@a,
  start angle/.store in=\dbp@anga,
  end point/.store in=\dbp@b,
  end angle/.store in=\dbp@angb,
  store/.store in=\dbp@storename,
  use store/.style={
    method=\dbp@get{#1}{method},
    first angle=\dbp@get{#1}{firstangle},
    last angle=\dbp@get{#1}{lastangle},
    middle param=\dbp@get{#1}{middleparam},
  },
  minimum radius/.code={
    \pgfmathsetmacro\dbp@radius{#1}
    \pgfmathsetmacro\dbp@rradius{#1}
    \pgfmathsetmacro\dbp@lradius{#1}
  },
  left and right minimum radii/.code args={#1 and #2}{
    \pgfmathsetmacro\dbp@lradius{#1}
    \pgfmathsetmacro\dbp@rradius{#2}
    \pgfmathsetmacro\dbp@radius{(\dbp@lradius + \dbp@rradius)/2}
  },
  method/.store in=\dbp@method,
  first angle/.store in=\dbp@firstangle,
  last angle/.store in=\dbp@lastangle,
  middle param/.store in=\dbp@midparam,
  reverse/.is if=dubinspathreverse,
}
\newcommand\dubinspathset[1]{\tikzset{dubins path,#1}}
\newcommand\dubinspathcalc[1]{%
  \begingroup
  \dubinspathset{#1}
  \tikzset{
    declare function={
      angtodist(\dbp@a,\dbp@r)={abs(\dbp@a)*.01745329*\dbp@r};
      modangr(\dbp@a,\dbp@b)={
        (
        Mod(\dbp@a,360)<Mod(\dbp@b,360)
        ?
        Mod(\dbp@a,360)
        :
        Mod(\dbp@a,360)-360)+\dbp@b-Mod(\dbp@b,360
        )
      };
      modangl(\dbp@a,\dbp@b)={
        (
        Mod(\dbp@a,360)<Mod(\dbp@b,360)
        ?
        Mod(\dbp@a,360)+360
        :
        Mod(\dbp@a,360))+(\dbp@b)-Mod(\dbp@b,360)
      };
    },
  }

  \pgfmathsetmacro\dbp@radius{\dbp@rradius}
  \pgfmathsetmacro\dbp@anga{mod((\dbp@anga)+180,360)-180}
  \pgfmathsetmacro\dbp@angb{mod((\dbp@angb)+180,360)-180}
  \path
  let
  \p{a}=(\dbp@a),
  \p{b}=(\dbp@b),
  \p{ar}=($(\p{a}) + (\dbp@anga-90:\dbp@radius pt)$),
  \p{al}=($(\p{a}) + (\dbp@anga+90:\dbp@radius pt)$),
  \p{br}=($(\p{b}) + (\dbp@angb-90:\dbp@radius pt)$),
  \p{bl}=($(\p{b}) + (\dbp@angb+90:\dbp@radius pt)$)
  in \pgfextra{
    \pgfinterruptpath

    % RSR (ar and br)
    \dbp@anglebetween\dbp@rsrarbr{\p{ar}}{\p{br}}
    \dbp@distancebetween\dbp@rsrdarbr{\p{ar}}{\p{br}}
    \pgfmathsetmacro\dbp@rsrangone{Mod(\dbp@anga-\dbp@rsrarbr,360)}
    \pgfmathsetmacro\dbp@rsrangtwo{Mod(\dbp@rsrarbr-\dbp@angb,360)}
    \pgfmathsetmacro\dbp@rsrlen{\dbp@rsrdarbr}
    \pgfmathsetmacro\dbp@rsrdist{
      angtodist(\dbp@rsrangone,\dbp@radius)
      +\dbp@rsrlen
      +angtodist(\dbp@rsrangtwo,\dbp@radius)
    }
    \dbp@setparams{rsr}{\dbp@rsrdist}{\dbp@rsrangone}{\dbp@rsrlen}{\dbp@rsrangtwo}

    % LSL (al and bl)
    \dbp@anglebetween\dbp@lslalbl{\p{al}}{\p{bl}}
    \dbp@distancebetween\dbp@lsldalbl{\p{al}}{\p{bl}}
    \pgfmathsetmacro{\dbp@lslangone}{mod(\dbp@lslalbl-\dbp@anga+720,360)}
    \pgfmathsetmacro{\dbp@lslangtwo}{mod(\dbp@angb-\dbp@lslalbl+720,360)}
    \pgfmathsetmacro\dbp@lsllen{\dbp@lsldalbl}
    \pgfmathsetmacro\dbp@lsldist{
      angtodist(\dbp@lslangone,\dbp@radius)
      +\dbp@lsllen
      +angtodist(\dbp@lslangtwo,\dbp@radius)
    }
    \dbp@updateparams%
    {lsl}{\dbp@lsldist}{\dbp@lslangone}{\dbp@lsllen}{\dbp@lslangtwo}

    % RSL (ar and bl)
    \dbp@distancebetween\dbp@rsldarbl{\p{ar}}{\p{bl}}
    \pgfmathtruncatemacro\dbp@rslok{(\dbp@rsldarbl>=2*\dbp@radius)?1:0}
    \ifnumequal{\dbp@rslok}{1}{
      \dbp@anglebetween\dbp@rslarbl{\p{ar}}{\p{bl}}
      \pgfmathsetmacro\dbp@rslanglesup{
        asin(\dbp@radius/\dbp@rsldarbl*2)}
      \pgfmathsetmacro\dbp@rslangone
      {Mod(\dbp@anga-\dbp@rslarbl+\dbp@rslanglesup,360)}
      \pgfmathsetmacro\dbp@rslangtwo
      {Mod(\dbp@angb-\dbp@rslarbl+\dbp@rslanglesup,360)}
      \pgfmathsetmacro\dbp@rsllen{veclen(\dbp@rsldarbl,\dbp@radius)}
      \pgfmathsetmacro\dbp@rsldist{
        angtodist(\dbp@rslangone,\dbp@radius)
        +\dbp@rsllen
        +angtodist(\dbp@rslangtwo,\dbp@radius)
      }

      \dbp@updateparams%
      {rsl}{\dbp@rsldist}{\dbp@rslangone}{\dbp@rsllen}{\dbp@rslangtwo}
    }{}

    % LSR (al and br)
    \dbp@distancebetween\dbp@lsrdalbr{\p{al}}{\p{br}}
    \pgfmathtruncatemacro\dbp@lsrok{(\dbp@lsrdalbr>=2*\dbp@radius)?1:0}
    \ifnumequal{\dbp@lsrok}{1}{
      \dbp@anglebetween\dbp@lsralbr{\p{al}}{\p{br}}
      \pgfmathsetmacro\dbp@lsranglesup{
        asin(\dbp@radius/\dbp@lsrdalbr*2)}
      \pgfmathsetmacro\dbp@lsrangone
      {Mod(\dbp@lsralbr+\dbp@lsranglesup-\dbp@anga,360)}
      \pgfmathsetmacro\dbp@lsrangtwo
      {Mod(\dbp@lsralbr+\dbp@lsranglesup-\dbp@angb,360)}
      \pgfmathsetmacro\dbp@lsrlen{veclen(\dbp@lsrdalbr,\dbp@radius)}
      \pgfmathsetmacro\dbp@lsrdist{
        angtodist(\dbp@lsrangone,\dbp@radius)
        +\dbp@lsrlen
        +angtodist(\dbp@lsrangtwo,\dbp@radius)
      }
      \dbp@updateparams%
      {lsr}{\dbp@lsrdist}{\dbp@lsrangone}{\dbp@lsrlen}{\dbp@lsrangtwo}
    }{}

    % LRL (al and bl)
    \dbp@distancebetween\dbp@lrldalbl{\p{al}}{\p{bl}}
    \pgfmathtruncatemacro\dbp@lrlok{(\dbp@lrldalbl<=4*\dbp@radius)?1:0}
    \ifnumequal{\dbp@lrlok}{1}{
      \dbp@anglebetween\dbp@lrlalbl{\p{al}}{\p{bl}}
      \pgfmathsetmacro\dbp@lrlangsup{acos(\dbp@lrldalbl/\dbp@radius/4)}
      \pgfmathsetmacro\dbp@lrlangone{
        modangl(\dbp@lrlalbl+\dbp@lrlangsup,\dbp@anga-90)-(\dbp@anga-90)}
      \pgfmathsetmacro\dbp@lrlangtwo{%
        (\dbp@angb-90)-modangr(\dbp@lrlalbl+180-\dbp@lrlangsup,\dbp@angb-90)}
      \pgfmathsetmacro\dbp@lrlangthree{360-2*(90-\dbp@lrlangsup)}
      \pgfmathsetmacro\dbp@lrldist{
        angtodist(\dbp@lrlangone,\dbp@radius)
        +angtodist(\dbp@lrlangthree,\dbp@radius)
        +angtodist(\dbp@lrlangtwo,\dbp@radius)
      }
      \dbp@updateparams%
      {lrl}{\dbp@lrldist}{\dbp@lrlangone}{\dbp@lrlangthree}{\dbp@lrlangtwo}
    }{}

    % RLR (ar and br)
    \dbp@distancebetween\dbp@rlrdarbr{\p{ar}}{\p{br}}
    \pgfmathtruncatemacro\dbp@rlrok{(\dbp@rlrdarbr<=4*\dbp@radius)?1:0}
    \ifnumequal{\dbp@rlrok}{1}{
      \dbp@anglebetween\dbp@rlrarbr{\p{ar}}{\p{br}}
      \pgfmathsetmacro\dbp@rlrangsup{acos(\dbp@rlrdarbr/\dbp@radius/4)}
      \pgfmathsetmacro\dbp@rlrangone{
        (\dbp@anga+90)-modangr(\dbp@rlrarbr-\dbp@rlrangsup,\dbp@anga+90)}
      \pgfmathsetmacro\dbp@rlrangtwo{%
        modangl(\dbp@rlrarbr+180+\dbp@rlrangsup,\dbp@angb+90)-(\dbp@angb+90)}
      \pgfmathsetmacro\dbp@rlrangthree{360-2*(90-\dbp@rlrangsup)}
      \pgfmathsetmacro\dbp@rlrdist{
        angtodist(\dbp@rlrangone,\dbp@radius)
        +angtodist(\dbp@rlrangthree,\dbp@radius)
        +angtodist(\dbp@rlrangtwo,\dbp@radius)
      }
      \dbp@updateparams%
      {rlr}{\dbp@rlrdist}{\dbp@rlrangone}{\dbp@rlrangthree}{\dbp@rlrangtwo}
    }{}

    \endpgfinterruptpath
  };
  \endgroup
}
\endinput
%%
%% End of file `tikzlibrarydubins.code.tex'.

